Efficient Low-rank Multimodal Fusion with Modality-Specific Factors

Multimodal research is an emerging field of artificial intelligence, and one of the main research problems in this field is multimodal fusion. The fusion of multimodal data is the process of integrating multiple unimodal representations into one compact multimodal representation. Previous research in this field has exploited the expressiveness of tensors for multimodal representation. However, these methods often suffer from exponential increase in dimensions and in computational complexity introduced by transformation of input into tensor. In this paper, we propose the Low-rank Multimodal Fusion method, which performs multimodal fusion using low-rank tensors to improve efficiency. We evaluate our model on three different tasks: multimodal sentiment analysis, speaker trait analysis, and emotion recognition. Our model achieves competitive results on all these tasks while drastically reducing computational complexity. Additional experiments also show that our model can perform robustly for a wide range of low-rank settings, and is indeed much more efficient in both training and inference compared to other methods that utilize tensor representations.

==> tables/iemocap.tex <==
\definecolor{gg}{RGB}{45,190,45}

\begin{table}[th!]
\fontsize{7.5}{10}\selectfont
%\centering
\setlength\tabcolsep{2.3pt}
\begin{tabular}{l : *{16}{K{0.673cm}}}
\Xhline{0.5\arrayrulewidth}
Dataset & \multicolumn{8}{c}{\textbf{IEMOCAP Emotions}} \\
Task & \multicolumn{2}{c}{Happy} & \multicolumn{2}{c}{Sad} & \multicolumn{2}{c}{Angry} & \multicolumn{2}{c}{Neutral} \\
%\cmidrule(lr{.5em}){2-3}  \cmidrule(lr{.5em}){4-5} \cmidrule(lr{.5em}){6-7} \cmidrule(lr{.5em}){8-9} 
Metric        	& A$^{2}$ & F1 & A$^{2}$ & F1 & A$^{2}$ & F1 & A$^{2}$ & F1 \\ 
\Xhline{0.5\arrayrulewidth}
SVM     		& 86.1 & 81.5 & 81.1 & 78.8 & 82.5 & 82.4 & 65.2 & 64.9 \\
% RF     			& 85.5 & 80.7 & 80.1 & 76.5 \\
TFN      		& 84.8 & 83.6 & 83.4 & 82.8 & 83.4 & 84.2 & 67.5 & 65.4 \\ 
DF   			& 86.0 & 81.0 & 81.8 & 81.2 & 75.8 & 65.4 & 59.1 & 44.0 \\
MV-LSTM   		& 85.9 & 81.3 & 80.4 & 74.0 & 85.1 & 84.3 & 67.0 & 66.7 \\
BC-LSTM    		& 84.9 & 81.7 & 83.2 & 81.7 & 83.5 & 84.2 & 67.5 & 64.1 \\
MARN			& 86.7 & 83.6 & 82.0 & 81.2 & 84.6 & 84.2 & 66.8 & 65.9 \\
MFN				& 86.5 & 84.0 & 83.5 & 82.1 & 85.0 & 83.7 & 69.6 & 69.2 \\
% \Xhline{0.5\arrayrulewidth}
{\ours}      & \textbf{87.3} & \textbf{85.8} & \textbf{86.2} & \textbf{85.9} & \textbf{89.0} & \textbf{89.0} & \textbf{72.4} & \textbf{71.7} \\ 
% \Xhline{0.5\arrayrulewidth}
% $\Delta_{SOTA}$	& \textcolor{gg}{$\uparrow $ \textbf{0.8}}  & \textcolor{gg}{\textbf{0.0}}  & \textcolor{gg}{$\uparrow $ \textbf{0.4}}  & \textcolor{gg}{$\uparrow $ \textbf{0.2}} & \textcolor{gg}{$\uparrow $ \textbf{0.6}} & \textcolor{gg}{$\uparrow $ \textbf{1.0}} & \textcolor{gg}{$\uparrow $ \textbf{0.6}} & \textcolor{gg}{$\uparrow $ \textbf{0.4}} \\ 
\Xhline{0.5\arrayrulewidth}
\end{tabular}
\caption{Emotion recognition results on IEMOCAP test set using multimodal methods. The best results are highlighted in bold.
% and $\Delta_{SOTA}$ shows the change in performance over previous state of the art. Improvements are highlighted in green. The \ours \ significantly outperforms the current state of the art across all evaluation metrics.
}
\label{table:iemocap}
\end{table}

==> tables/mmmo.tex <==
\begin{table*}[!h]
\fontsize{7}{10}\selectfont
%\centering
\setlength\tabcolsep{1.3pt}
\begin{tabular}{l : *{16}{K{1.09cm}}}
\Xhline{3\arrayrulewidth}
%Dataset    &  \multicolumn{4}{c:}{ICT-MMMO}  \\
Task		& \multicolumn{4}{c:}{\textbf{ICT-MMMO Sentiment}} \\
Metric       & BA & F1 & MAE & $r$  \\ \Xhline{0.5\arrayrulewidth}
{TFN } 	 & 72.5	& 72.6 & - & - \\ 
{MARN } 	 & 86.3	& 85.9 & - & - \\
{MFN } 	 & \textbf{87.5}	& \textbf{87.1} & \textbf{0.739} & \textbf{0.696}  \\ 
{\ours } 	 & 82.5	& 82.6 & 0.884 & 0.573  \\ 
\Xhline{0.5\arrayrulewidth}
% $\Delta_{SOTA}$	& \textcolor{gg}{$\downarrow $ \textbf{0.103}} & \textcolor{gg}{$\uparrow $ \textbf{0.108}} & \textcolor{gg}{$\uparrow $ \textbf{10.8}} & \textcolor{gg}{$\uparrow $ \textbf{9.9}} & \textcolor{gg}{$\uparrow $ \textbf{7.1}} & \textcolor{gg}{$\uparrow $ \textbf{5.7}} \\ \Xhline{3\arrayrulewidth}
\end{tabular}
\label{tables:mmmo}
\end{table*}

==> tables/mosi.tex <==
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
\definecolor{gg}{RGB}{45,190,45}
\definecolor{gray}{RGB}{128, 128, 128}

\begin{table}[hb!]
\fontsize{7.5}{10}\selectfont
%\centering
\setlength\tabcolsep{3pt}
\begin{tabular}{l : *{16}{K{1.1cm}}}
\Xhline{0.5\arrayrulewidth}
Dataset & \multicolumn{5}{c}{\textbf{CMU-MOSI}} \\
Task & \multicolumn{5}{c}{Sentiment} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Metric        & MAE & Corr & A$^{2}$ & F1 & A$^{7}$\\ 
\Xhline{0.5\arrayrulewidth}

DF              & 72.3 &   72.1   &  26.8 	& 1.143     &  0.518 \\
MV-LSTM			& 73.9 &   74.0   &  33.2	& 1.019 &  0.601 \\
BC-LSTM         & 73.9 &   73.9   &  28.7	& 1.079 &  0.581 \\ 
TFN            	& 0.970	& 0.633   & 73.9 &   73.4   &  32.1 \\ 
%GME-LSTM(A) & 0.955 & - & 76.5 & 73.4 & - \\
MARN  & 0.968  & 0.625 & 77.1	& 77.0 & 34.7\\ 
MFN  	&  {0.965}    	& {0.632} & {\textbf{77.4}}	 & {\textbf{77.3}}   & {\textbf{34.1}}\\
\Xhline{0.5\arrayrulewidth}
{\ours}			& \textbf{0.912}	&	\textbf{0.668} & 76.4	& 75.7	& 32.8 \\
% \Xhline{0.5\arrayrulewidth}
% $\Delta_{SOTA}$	 & \textcolor{gg}{$\downarrow $ \textbf{0.043}} & \textcolor{gg}{$\uparrow $ \textbf{0.004}} & \textcolor{gray}{$\downarrow $ \textbf{1.3}} & \textcolor{gray}{$\downarrow $ \textbf{2}} & \textcolor{gray}{$\downarrow $ \textbf{2.8}} \\ 
% \Xhline{0.5\arrayrulewidth}
% Human & 85.7 &   87.5   &  53.9	&    0.710    	&  0.820  \\
\Xhline{0.5\arrayrulewidth}
\end{tabular}
\caption{Sentiment prediction results on the CMU-MOSI test set using multimodal methods.
% The {\ours} achieves better performance on MAE and Corr metrics compared to the previous state-of-the-art models. 
The best results are highlighted in bold.
% and $\Delta_{SOTA}$ shows the change in performance over previous state of the art. Improvements are highlighted in green. 
}
\label{table:mosi}
\end{table}

==> tables/pom.tex <==
\definecolor{gg}{RGB}{45,190,45}
\definecolor{gray}{RGB}{128, 128, 128}

\begin{table*}[th!]
\fontsize{7}{10}\selectfont
%\centering
\setlength\tabcolsep{1.3pt}
\begin{tabular}{p{1.2cm} : *{17}{K{0.77cm}}}
\Xhline{0.5\arrayrulewidth}
Dataset & \multicolumn{17}{c}{\textbf{POM}} \\
Task & \multicolumn{1}{c}{Con} & \multicolumn{1}{c}{Pas} & \multicolumn{1}{c}{Voi} & \multicolumn{1}{c}{Dom} & \multicolumn{1}{c}{Cre} & \multicolumn{1}{c}{Viv} & \multicolumn{1}{c}{Exp} & \multicolumn{1}{c}{Ent} & \multicolumn{1}{c}{Res} & \multicolumn{1}{c}{Tru} & \multicolumn{1}{c}{Rel} & \multicolumn{1}{c}{Out} & \multicolumn{1}{c}{Tho} & \multicolumn{1}{c}{Ner} & \multicolumn{1}{c}{Per} & \multicolumn{1}{c}{Hum} & \multicolumn{1}{c}{Avg}\\
Metric & A$^7$ & A$^7$ & A$^7$ & A$^7$ & A$^7$ &  A$^7$ &  A$^7$ &  A$^7$ & A$^5$ & A$^5$ & A$^5$ & A$^5$ &  A$^5$ &  A$^5$ & A$^7$ & A$^5$ & A \\ 
\Xhline{0.5\arrayrulewidth}
SVM     		&  20.6 & 20.7 & 32.0 & 35.0 & 25.1 & 29.1 & 26.6 & 31.5 & 34.0 & 50.2 & 49.8 & 42.9 & 39.9 & 41.4 & 28.1 & 36.0 \\
% RF     			&  26.6&27.1&29.6&26.1&23.2&23.6&26.6&26.1&34.0&53.2&40.9&32.5&37.4&36.0&25.6&40.4  \\
TFN & 24.1&31.0&31.5&34.5&24.6&25.6&27.6&29.1&30.5&38.9&35.5&37.4&33.0&42.4&27.6&33.0 & 31.6\\
DF   & 25.6&24.1&33.0&34.0&26.1&32.0&26.6&29.6&30.0&53.7&50.2&39.4&37.9&42.4&26.6&34.5\\
MV-LSTM 		& 25.6&28.6&28.1&34.5&25.6&32.5&29.6&29.1&33.0&52.2&50.7&38.4&37.9&42.4&26.1&38.9\\
BC-LSTM    		& 26.6&26.6&31.0&33.0&27.6&36.5&30.5&29.6&33.0&52.2&47.3&37.9&45.8&36.0&27.1&36.5\\ 
MARN 	&  
29.1&33.0& -&38.4&31.5& -& -&33.5&36.9&55.7&52.2&-& -& 47.3&31.0&44.8 & 39.4\\ 
MFN 	& 
34.5&35.5&\textbf{37.4}&\textbf{41.9}&34.5&36.9&36.0&37.9&38.4&57.1&\textbf{53.2}&46.8&47.3&47.8&\textbf{34.0}&47.3 & 41.7\\ 

\Xhline{0.5\arrayrulewidth}

{\ours } 	& 
\textbf{36.9}&\textbf{36.5}&\textbf{37.4}&41.4&\textbf{36.5}&\textbf{38.9}&\textbf{40.4}&\textbf{39.9}&\textbf{39.9}&\textbf{58.6}&\textbf{53.2}&\textbf{48.3}&\textbf{48.8}&\textbf{50.2}&32.0&\textbf{45.8} & \textbf{42.8}\\ 
\Xhline{0.5\arrayrulewidth}
\end{tabular}
\\
\\
\\
\begin{tabular}{p{1.2cm} : *{17}{K{0.77cm}}}
\Xhline{0.5\arrayrulewidth}

Metric & \multicolumn{17}{c}{MAE} \\ 
Task & \multicolumn{1}{c}{Con} & \multicolumn{1}{c}{Pas} & \multicolumn{1}{c}{Voi} & \multicolumn{1}{c}{Dom} & \multicolumn{1}{c}{Cre} & \multicolumn{1}{c}{Viv} & \multicolumn{1}{c}{Exp} & \multicolumn{1}{c}{Ent} & \multicolumn{1}{c}{Res} & \multicolumn{1}{c}{Tru} & \multicolumn{1}{c}{Rel} & \multicolumn{1}{c}{Out} & \multicolumn{1}{c}{Tho} & \multicolumn{1}{c}{Ner} & \multicolumn{1}{c}{Per} & \multicolumn{1}{c}{Hum} & \multicolumn{1}{c}{Avg}\\
\Xhline{0.5\arrayrulewidth}
SVM	& 1.071&1.159&0.938&0.865&1.036&1.043&1.031&0.988&0.877&0.536&0.594&0.702&0.728&0.714&1.110&0.801\\
TFN & 1.049&1.104&0.927&0.864&1.058&1.000&1.029&0.973&0.900&0.572&0.621&0.706&0.743&0.727&1.132&0.770 & 0.886\\
DF & 1.033&1.083&0.899&0.870&1.039&0.997&1.027&0.967&0.884&0.534&0.591&0.698&0.732&0.695&1.086&0.768 \\
MV-LSTM	& 	1.029&1.098&0.971&0.944&1.082&0.976&1.012&0.998&0.877&0.523&0.625&0.703&0.792&0.687&1.163&0.770 \\
BC-LSTM		& 1.016&1.008&0.914&0.859&0.942&0.905&0.906&0.927&0.888&0.564&0.630&0.708&0.680&0.705&1.025&0.767	 \\
{MFN } 	& 
0.952&0.993&0.882&0.835&\textbf{0.903}&0.908&\textbf{0.886}&0.913&0.821&0.521&0.566&0.679&\textbf{0.665}&\textbf{0.654}&\textbf{0.981}&0.727 & 0.805 \\ 

\Xhline{0.5\arrayrulewidth}

{\ours } 	& 
\textbf{0.900}&\textbf{0.945}&\textbf{0.848}&\textbf{0.827}&0.946&\textbf{0.903}&0.885&\textbf{0.882}&\textbf{0.805}&\textbf{0.516}&\textbf{0.564}&\textbf{0.654}&0.674&0.655&1.017&\textbf{0.718} & \textbf{0.796} \\ 
\Xhline{0.5\arrayrulewidth}
\end{tabular}
\\
\\
\\
\begin{tabular}{p{1.2cm} : *{17}{K{0.77cm}}}
\Xhline{0.5\arrayrulewidth}
Metric  & \multicolumn{17}{c}{Corr}  \\ 
Task & \multicolumn{1}{c}{Con} & \multicolumn{1}{c}{Pas} & \multicolumn{1}{c}{Voi} & \multicolumn{1}{c}{Dom} & \multicolumn{1}{c}{Cre} & \multicolumn{1}{c}{Viv} & \multicolumn{1}{c}{Exp} & \multicolumn{1}{c}{Ent} & \multicolumn{1}{c}{Res} & \multicolumn{1}{c}{Tru} & \multicolumn{1}{c}{Rel} & \multicolumn{1}{c}{Out} & \multicolumn{1}{c}{Tho} & \multicolumn{1}{c}{Ner} & \multicolumn{1}{c}{Per} & \multicolumn{1}{c}{Hum} & \multicolumn{1}{c}{Avg}\\
\Xhline{0.5\arrayrulewidth}
SVM	& 0.063&0.086&-0.004&0.141&0.113&0.076&0.134&0.141&0.166&0.168&0.104&0.066&0.134&0.068&0.064&0.147\\
TFN &  0.089&0.201&0.030&0.020&0.124&0.204&0.171&0.223&-0.051&-0.064&0.114&0.060&0.048&-0.002&0.106&0.213 & 0.093 \\ 
DF	& 0.240&0.273&0.017&0.139&0.112&0.173&0.118&0.217&0.148&0.143&0.019&0.093&0.041&0.136&0.168&0.259 \\
MV-LSTM	& 0.358&0.416&0.131&0.146&0.280&0.347&0.323&0.326&0.295&0.237&0.119&0.238&0.284&0.258&0.239&0.317 \\
BC-LSTM & 0.359&0.425&0.081&0.234&0.358&0.417&0.450&0.361&0.293&0.109&0.075&0.078&0.363&0.184&0.344&0.319\\
MFN & 
0.395&0.428&0.193&0.313&0.367&0.431&0.452&0.395&0.333&\textbf{0.296}&0.255&0.259&\textbf{0.381}&0.318&\textbf{0.377}&0.386 & 0.349\\ \Xhline{0.5\arrayrulewidth}

{\ours }  &  \textbf{0.481}&\textbf{0.502}&\textbf{0.271}&\textbf{0.447}&\textbf{0.408}&\textbf{0.439}&\textbf{0.479}&\textbf{0.433}&\textbf{0.418}&0.245&\textbf{0.272}&\textbf{0.407}&0.370&\textbf{0.375}&0.353&\textbf{0.432} & \textbf{0.396}\\ 
\Xhline{0.5\arrayrulewidth}
\end{tabular}
\caption{Results for personality trait recognition on POM. The last column of the table indicates the average accuracy over 16 personality traits. Best results are highlighted in bold. 
}
\label{table:pom}
\end{table*}
